DreamTalk: When Emotional Talking Head Generation Meets Diffusion Probabilistic Models

Emotional talking head generation has attracted growing attention. Previous methods, which are mainly GAN-based, still struggle to consistently produce satisfactory results across diverse emotions and cannot conveniently specify personalized emotions. In this work, we leverage powerful diffusion models to address the issue and propose DreamTalk, a framework that employs meticulous design to unlock the potential of diffusion models in generating emotional talking heads. Specifically, DreamTalk consists of three crucial components: a denoising network, a style-aware lip expert, and a style predictor. The diffusion-based denoising network can consistently synthesize high-quality audio-driven face motions across diverse emotions. To enhance lip-motion accuracy and emotional fullness, we introduce a style-aware lip expert that can guide lip-sync while preserving emotion intensity. To more conveniently specify personalized emotions, a diffusion-based style predictor is utilized to predict the personalized emotion directly from the audio, eliminating the need for extra emotion reference. By this means, DreamTalk can consistently generate vivid talking faces across diverse emotions and conveniently specify personalized emotions. Extensive experiments validate DreamTalk's effectiveness and superiority. The code is available at https://github.com/ali-vilab/dreamtalk.

==> sec/0_abstract.tex <==
\begin{abstract}
Emotional talking head generation has attracted growing attention.
%
Previous methods, which are mainly GAN-based, still struggle to consistently produce satisfactory results across diverse emotions and cannot conveniently specify personalized emotions.
%
In this work, we leverage powerful diffusion models to address the issue and propose DreamTalk, a framework that employs meticulous design to unlock the potential of diffusion models in generating emotional talking heads.
%
Specifically, DreamTalk consists of three crucial components: a denoising network, a style-aware lip expert, and a style predictor.
%
The diffusion-based denoising network can consistently synthesize high-quality audio-driven face motions across diverse emotions.
%
To enhance lip-motion accuracy and emotional fullness, we introduce a style-aware lip expert that can guide lip-sync while preserving emotion intensity. 
% 
To more conveniently specify personalized emotions, a diffusion-based style predictor is utilized to predict the personalized emotion directly from the audio, eliminating the need for extra emotion reference.
%
By this means, DreamTalk can consistently generate high-quality talking faces across diverse emotions and conveniently specify personalized emotions.
%
Extensive experiments validate DreamTalk's effectiveness and its superiority over state-of-the-art methods. Code and models will be released.
  \keywords{Emotional talking head generation \and Diffusion models}
\end{abstract}

==> supp_sec/01_additional_evaluation_for_speaking_style_prediction.tex <==
\section{Additional Evaluation for Speaking Style Prediction}
\label{sec:additional_evaluation_for_speaking_style_prediction}

\subsection{Ablation Study}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/style_predictor_ablation.pdf}
  % \vspace{-3mm}
  \caption{The qualitative results of style predictor's ablation study.}
  % \vspace{-2mm}
  \label{fig:style_predictor_ablation}
  % \vspace{-0.1cm}
\end{figure}


% To analyze the contributions of our designs, we conduct an ablation study with three variants: (1) remove the speaker information input and only use audio to predict (\textbf{w/o speaker info}); (2) during model training, the speaker info and audio are both obtained from the same video (\textbf{w/o cross-ID training}); (3) predict using regression model instead of diffusion model (\textbf{regression}). Our full model is denoted as \textbf{Full}. When generating samples for evaluation, the facial images and audio we use are sourced from videos of the same individual expressing different emotions. This generation approach better aligns with real-world applications.   

To evaluate the impact of our design choices, we conduct an ablation study with three variants: (1) omitting speaker information and relying solely on audio for prediction (\textbf{w/o speaker info}); (2) during model training, the speaker info and audio are both obtained from the same video (\textbf{w/o cross-ID training}); (3) employing a regression model instead of a diffusion model for prediction (\textbf{regression}). Our full model is denoted as \textbf{Full}. When generating samples for evaluation, the facial images and audio we use are sourced from videos of the same individual expressing different emotions(\textit{e. g.} the face image is from a happy video while the audio is from an angry one.). This generation approach better aligns with real-world applications.   

% The findings are detailed in \cref{table:style_predictor_ablation_study} and \cref{fig:style_predictor_ablation}.

How to quantitatively evaluate the performance of speaking style prediction has not been explored before. we devise three metrics:
\begin{itemize}
    \item \textbf{Style Code Distance (SCD)} We extract the style codes from the videos that provide the audio input and compute the L2 distance between the predicted style codes and these style codes.
    \item \textbf{Motion Distance (MD)} We use the predicted style codes and the audio used for prediction to generate face motions and compute the L2 distance between the generated face motions and the face motions extracted from the ground truth videos. 
    \item \textbf{Style Accuracy (SA)} We use the SA metric mentioned in the main paper. SA is evaluated on 3DMM face motions. The details of SA are reported in \cref{sec:style_accuracy_metric}. The ground truth testing set gets $92.5\%$ accuracy.
\end{itemize}
% We do not devise metrics on image level (\eg train a image classifier to classify speaking style) for the following reasons: first, the expression-irrelevant information, such as speaker, and background, will interfere with the prediction of nuanced speaking style. Second, the error caused by renderer also interfere with the prediction of nuanced speaking style.
We refrain from devising image-level metrics, such as training an image classifier for speaking style classification, due to several critical considerations. Firstly, factors in images that are irrelevant to expression, such as the speaker's identity and background elements, can adversely impact the accurate prediction of nuanced speaking styles. Secondly, inaccuracies introduced by the rendering process may further additionally hinder the accurate discernment of these subtle speaking styles.

\begin{table}[t]
% \small
\centering
\setlength{\tabcolsep}{3.5mm}{
\begin{tabular}{cccc}
% \toprule  
Method & SCD$\downarrow$ & MD$\downarrow$ & SA$\uparrow$  \\
% \midrule
\shline
w/o speaker info   & 0.49 & 0.28 & 64.3  \\
w/o cross-ID training  & 0.68 & 0.45 & 28.1  \\
regression  & 0.56 & 0.32 & 55.1 \\
\textbf{Full} & \textbf{0.42}  &  \textbf{0.23} & \textbf{78.6} \\

% \bottomrule 
\end{tabular}}
\vspace{-3mm}
\caption{The ablation study results of the style predictor.}
\vspace{-4mm}
\label{table:style_predictor_ablation_study}
\end{table}

% The results are shown in \cref{table:style_predictor_ablation_study} and \cref{fig:style_predictor_ablation}.
% \textbf{w/o speaker info} can predict correct emotions from audio, but occasionally the predicted speaking style is not consistent with the speaker identity, which leads to bad identity preservation. This demonstrates that speaker information aids in predicting speaking styles. Although in experiments, we observed that \textbf{w/o cross-ID training} achieves slightly better performance than \textbf{Full} when the input portrait and audio are from the same video, \textbf{w/o cross-ID} perform worse (cannot even predict the correct emotion) when the input portrait and audio are from the different videos. This indicates that the identity 3DMM parameters still contain some expression information and without cross-ID training, the model may infer the emotion from the leaked information instead of the audio. \textbf{regression} fails to generate correct expressions for some data. This indicates that the great distribution-learning property of diffusion models aids the speaking style prediction.

The results are shown in \cref{table:style_predictor_ablation_study} and \cref{fig:style_predictor_ablation}.
The \textbf{w/o speaker info} variant successfully predicts emotions from audio but occasionally fails to maintain consistency between the predicted speaking style and speaker identity, leading to poor identity preservation. This underscores the importance of speaker information in predicting speaking styles. Although in experiments, we observed that \textbf{w/o cross-ID training} achieves slightly better performance than \textbf{Full} when the input portrait and audio are from the same video, it underperformed, often failing to predict the correct emotion, when inputs were from different videos. This suggests that identity 3DMM parameters may convey some expression information, and without cross-ID training, the model might derive emotional cues from this leaked information rather than the audio. The \textbf{regression} variant struggles to generate accurate expressions for certain data, highlighting the superior distribution-learning capability of diffusion models in facilitating speaking style prediction.


% , but achieves lower performance than \textbf{Full},

\subsection{User Study}
In our user study, we evaluate the alignment between the original and predicted speaking styles. 
Directly assessing the alignment of speaking styles can be somewhat ambiguous, so we employ a comparative approach for evaluation.
Specifically, we create a series of video triplets. Each triplet consisted of a test video from our dataset and two generated videos. 
The first video was generated using a style code predicted from an input portrait, sharing the same speaker identity as in the test video but displaying a neutral emotion, combined with the audio from the test video. The second video is generated using the style code extracted from videos with the same emotion but from a speaker different from the one in the test video. We recruit 20 participants. Each participant is then asked to evaluate 20 triplets and identify which of the generated videos most accurately reflected the speaking style of the test video. 
The videos generated using predicted style codes are preferred in $75.8\%$ of all ratings. This indicates that the style predictor is able to infer personalized speaking styles that are aligned with the audio. 

\subsection{Analyzing the Influence of Portraits}


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/influence_of_portraits.pdf}
  % \vspace{-3mm}
  \caption{Analyzing the influence of portraits on style prediction. The audio conveys surprised emotion.}
  % \vspace{-2mm}
  \label{fig:influence_of_portraits}
  % \vspace{-0.1cm}
\end{figure}

We analyze the influence of portraits on speaking style prediction by predicting speaking styles with an audio clip and different input portraits. The predicted styles are subsequently applied to an identical portrait for a clearer comparison. As shown in \cref{fig:influence_of_portraits}, the predicted speaking styles match the subtle identity characteristics, such as gender, of the input portraits. The predicted style A generated more feminine results. This validates the necessity of integrating portrait information during style prediction.

==> supp_sec/02_additional_results_for_expressive_talking_head_generation.tex <==
\section{Additional Results for Emotional Talking Head Generation}

\subsection{Analysis on Generalization Capabilities}
\label{sec:analysis_on_generalization_capabilities}

\noindent\textbf{Songs.}
As demonstrated in \suppvideo, our method successfully generates reasonable results for songs, even those with accompaniment, despite this being significantly different from the training dataset's data distribution. A noticeable decline in lip-sync accuracy is observed when the accompaniment volume is excessively high. We conduct a comparative analysis of lip-sync performance between songs with accompaniment and songs with removed accompaniment (using data from the SingFace Dataset~\cite{liu2023musicface}). It is found that the accompaniment adversely affects lip-sync, leading to mouth movements resembling mumbling. Addressing the negative impact of accompaniment on lip-sync accuracy presents an interesting avenue for future research.
% As shown in \suppvideo, our method is able to generate reasonable results for songs even with accompaniment, which is far from the data distribution of the training dataset. We observe a performance drop on lip-sync when the accompaniment is too loud. We compare the lip-sync performance of results generated using Songs with accompaniment and Songs with the accompaniment removed (from SingFace Dataset~\cite{liu2023musicface}) and observe that the accompaniment compromises the lip-sync, dragging the mouth to mumbling motions. How to reduce the adverse effect of accompaniment on lip-sync is leaved for future research.

\noindent\textbf{Speech in Multiple Languages.}
\suppvideo shows that our method generates satisfactory results with speech in French, Chinese, Spanish, German, Italian, Japanese, and Korean. The versatility of wav2vec features aids application across various languages. Additionally, the inclusion of multilingual talking head videos from Voxceleb2 enhances generalization.
% The supplementary video demonstrates that our method effectively generates results with French, Chinese, Spanish, Italian, Japanese, and Korean speech. Wav2vec's versatile features enable application across various languages. 

\noindent\textbf{Noisy Audio.}
% \suppvideo shows that our method generates satisfactory results with audio that is noised with different types of noise and different noise intensity levels.
% We use the noise recorded in a meeting, in the office and in the cafeteria, which are the common environment for talking head applications,  from DEMAND dataset~\cite{thiemann2013diverse} and mix the audio with noise using an off-the-shelf software \footnote{\url{https://github.com/Sato-Kunihiko/audio-SNR}} at SNR 20dB, 10dB, and 0dB. We observe no noticeable performance drop even at 0dB, where the noise is as loud as the speech and causes a significant decrease in the intelligibility and clarity of the speech.
\suppvideo demonstrates that our method yields satisfactory outcomes when processing audio mixed with multiple noise types and intensities. We employ noise recordings from typical talking head application environments—meetings, offices, and cafeterias—sourced from the DEMAND dataset~\cite{thiemann2013diverse}. We blend the audio with noise at several SNRs and test the performance. We found that our method maintains performance even at 0 dB SNR, where the noise is as loud as the speech and significantly impairs speech intelligibility and clarity.




\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/compare_with_diffused_head.pdf}
  % \vspace{-3mm}
  \caption{Comparisons with Diffused Head. Diffused Head frequently generate distorted faces and warped images.}
  \label{fig:compare_with_diffused_head}
  % \vspace{-2mm}
  % \vspace{-0.1cm}
\end{figure}

\subsection{More Comparisons with Diffused Head and TH-PAD}
We compare our method with Diffused Head~\cite{stypulkowski2023diffused} and TH-PAD~\cite{yu2023talking}, two diffusion-based methods,  on MEAD. For a fair comparison, we use audio to specify the styles used by DreamTalk. \cref{table:compare_with_thpad_dh} shows that DreamTalk achieves the best scores. 
The expressions produced by TH-PAD only synchronize with the audio rhythm but do not match the audio's emotion. Although TH-PAD is also trained on datasets with emotional expressions, TH-PAD focuses on expression diversity but does not consider the alignment with the audio's emotional content, while achieving emotional alignment is a more difficult task. We also observe that TH-PAD often changes the speaker identity. Diffused Head can only generate discrete types of emotions and cannot control the personalized variations of emotions. It also frequently generates distorted faces and warped images, shown in \cref{fig:compare_with_diffused_head}, which may be due to the buildup of errors across the sequence of generated frames.

\begin{table}[t]
% \small
\centering
\caption{Comparisons with Diffused Head and TH-PAD. DreamTalk(A) uses styles inferred from audio.}
\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{cccccc}
% \toprule  
Method & SSIM$\uparrow$ & CPBD &F/M-LMD$\downarrow$ & SA$\uparrow$ & $\text{Sync}_{\text{conf}}$$\uparrow$ \\
% \midrule
\shline
Diffused Head   & 0.54 & 0.08 & 5.61/6.85 &  22.6  &  1.87 \\

TH-PAD & 0.46 & 0.05 & 6.38/5.81 & 5.3 & 2.42 \\

\textbf{DreamTalk(A)}  & \textbf{0.84} & \textbf{0.16} & \textbf{2.24}/\textbf{3.43} &  \textbf{78.6}  & \textbf{3.73}\\

\textcolor{gray}{GT} & \textcolor{gray}{1} &  \textcolor{gray}{0.22} & \textcolor{gray}{0}/\textcolor{gray}{0} & \textcolor{gray}{92.5} & \textcolor{gray}{4.13} \\ 

% \bottomrule 
\end{tabular}}


\label{table:compare_with_thpad_dh}
\end{table}

\subsection{More ablation studies}

\begin{table}[t]
% \small
\centering
\caption{The additional results of DreamTalk's ablation study on MEAD.}
\setlength{\tabcolsep}{0.5mm}{
\begin{tabular}{ccccc}
% \toprule  
Method & SSIM$\uparrow$ & F-LMD$\downarrow$ & M-LMD$\downarrow$  & $\text{Sync}_{\text{conf}}$$\uparrow$ \\
% \midrule
\shline
% w/o Lip Expert   & 0.85 & \textbf{1.90} & 3.07   &  2.63 \\
% Uncond Lip Expert  & 0.83 & 2.19 & 3.42    & \textbf{4.51}\\
w/o Diffusion  & 0.82 & 2.25 & 3.39    & 3.18 \\
Blend. Lip Expert  & 0.83 & 2.10 & 3.03    & 3.32 \\
% \cmidrule(r){1-5}
\textbf{Full} & \textbf{0.86}  &  \textbf{1.93} & \textbf{2.91}   & \textbf{3.78} \\

% \bottomrule 
\end{tabular}}



\label{table:more_ablation_study}
\end{table}

To further validate the effectiveness of our design, we conduct an ablation study with two variants: (1) replace the diffusion model with a GAN model that uses the same architecture but is trained using GAN loss and regression loss(\textbf{w/o Diffusion}); (2) use the 3DMM expression parameters (blendshapes) as the input of lip expert, instead of using only the vertices in the mouth area(\textbf{Blend. Lip Expert}).

\cref{table:more_ablation_study} shows the results. \textbf{w/o Diffusion} cannot consistently generate correct emotional expressions and accurate lip-sync for diverse speaking styles (\suppvideo shows an example), potentially due to GAN's mode-collapse issue. Its scores are all lower than \textbf{Full}. This validates diffusion models' superiority over GANs in emotional talking head generation. \textbf{Blend. Lip Expert} also has degraded performance in generating emotional expressions and lip-sync. This is because, within the blendshapes, information about the mouth shape is mixed with that of other facial features. Therefore, when training a lip expert with blendshapes as input, information from other parts of the face can interfere with the accurate judgment of mouth shapes. The result validates the necessity of using mouth vertices as the input for the lip expert.




\subsection{Style Code Interpolation.}
\label{sec:style_code_interpolation}
Leveraging the style space, we can modify speaking styles via style code manipulation. \cref{fig:interpolation} illustrates that linear interpolation between style codes results in a seamless transition of generated speaking styles. This interpolation process allows for style intensity modulation and the generation of novel speaking styles.


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/interpolation.pdf}
  % \vspace{-3mm}
  \caption{The results of speaking style interpolation.}
  \label{fig:interpolation}
  % \vspace{-2mm}
  % \vspace{-0.1cm}
\end{figure}

\subsection{More Results of Style Code Visualization}
\label{sec:more_results_of_style_code_visualization}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/personalized_style_code_visualization.pdf}
  % \vspace{-4mm}
  \caption{t-SNE visualization of style codes for 3 speakers, with darker hues representing increased emotional intensity.}
  \label{fig:personalized_style_code_visualization}
  % \vspace{-0.1cm}
\end{figure}
We observe that each speaker's style code distribution exhibits both common patterns and individualized characteristics. Common patterns include: Firstly, speaking styles of different emotions cluster together first, with styles of lower intensity being closer to neutral and those of higher intensity being further away. Secondly, speaking styles of anger and disgust, as well as fear and surprise, often cluster together, as shown in \cref{fig:personalized_style_code_visualization}~(b) and (c).  Note that unlike \cite{ma2023styletalk}, our method does not incorporate losses to constrain style space.


\cref{fig:personalized_style_code_visualization}~(a) illustrates an example of individualized characteristics. The speaker's manifestation of fear closely resembles sadness, lacking the characteristic wide-eyed and open-mouthed expression, thereby positioning the speaking styles of fear nearer to those of sadness rather than surprise. Even within the same emotion, a speaker's speaking style can exhibit notable variation.
In \cref{fig:personalized_style_code_visualization}~(c), the speaker's dual expression of sadness—once with clenched teeth, similar to happy expressions, and another with depressed lip corners, akin to disgust—results in style codes close to the respective emotions. This observation diminishes the rationale for manually categorizing styles based on emotion and intensities in \cite{ma2023styletalk}.


\subsection{Generating emotions with personalized variations}

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/personalized_emotion.pdf}
  % \vspace{-4mm}
  \caption{DreamTalk can generate emotions with personalized variations.}
  \label{fig:personalized_emotions}
  % \vspace{-0.1cm}
\end{figure}

As shown in \cref{fig:personalized_emotions}, different persons express a single type of emotion with different expressions, and DreamTalk can generate emotions with such personalized variations. Fear style A conveys the emotion through narrowed eyes, whereas style B manifests it with eyes and mouth wide open. DreamTalk accurately generated the corresponding facial expressions.



% \subsection{Discussions Regarding Diffusion-based Methods}

% Recently, a few talking head generation methods~\cite{tian2024emo,stypulkowski2023diffused,shen2023difftalk,yu2023talking,du2023dae} have started to explore the use of diffusion models.
% Most methods utilize diffusion models to directly generate the image pixels, while DreamTalk adopts a different approach: it first uses diffusion models to generate audio-driven facial motions and then converts the motions into images. This design is based on our belief that learning the mappings from audio to motion and from motion to image separately is easier than directly learning the mapping from audio to image. An audio segment is more closely related to the facial motions, such as the opening and closing of the mouth, and less related to the specific colors of image pixels, such as black or white. Although such a two-stage design's performance may be limited by the expressiveness of the face representation~\cite{tian2024emo}, the ease of learning facilitates the model to learn accurate and vivid face motions. The advantage is more important for emotional talking head generation since it is a more severe one-to-many mapping problem and hence is more challenging to learn. The two-stage design eases the learning difficulty and hence allows DreamTalk to achieve high-quality results across diverse emotions.

==> supp_sec/03_implementation_details.tex <==
\section{Implementation Details}

\subsection{Architectual Details}

\subsubsection{Denoising Network} The audio encoder processes an input window of 11 sequential audio features, each of dimension $1024$. These features undergo dimension reduction to $256$ via a linear layer and then are fed to a transformer encoder comprising three 8-head transformer encoder layers, each with a hidden size of 256. Subsequently, a linear layer transforms the output tokens to yield audio tokens sized $11 \times 256$. The audio tokens are concatenated with noisy motion and then added with the encoded diffusion step.

The style encoder ingests sequential expression parameters from style reference videos, each sequence sized $N \times 64$. These sequences, ranging in length from 64 to 256 frames, are initially expanded to 256 dimensions via a linear layer. Subsequently, they are introduced into a transformer encoder, composed of three 8-head layers, each with a hidden size of 256. The resulting output tokens, each with a dimension of $256$, are aggregated through self-attention pooling~\cite{safari2020self}, yielding a style code of dimension $256$.

Within the decoder, the style code is repeated $11$ times, subsequently added with positional embedding to produce style tokens. These tokens, in conjunction with audio tokens, are processed by a transformer decoder, encompassing three 8-head layers, each with a hidden dimension of 256. Here, style tokens serve as the query, while audio tokens serve as both key and value. The middle output token is fed into a linear layer to predict facial motion.

% For implementation, inspired by ~\citet{ma2023styletalk}, we segregate expression parameters into lower and upper facial groups. Two parallel decoders are then employed to predict their respective groups. The resultant outputs are combined to derive the final facial motion.

\subsubsection{Style-aware Lip Expert}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.47\textwidth]{figures/lip_expert_architecture.pdf}
  % \vspace{-3mm}
  \caption{The architecture of mouth embedder and audio embedder. ConvBlock consists of a 1D CNN layer, a batch normalization layer, and a ReLU layer. "k3, 32, s2" means that the kernel size is 3, the output dimension is 32, and the stride is 2. ConvRBlock is a ConvBlock with residual connection.}
  % \vspace{-2mm}
  \label{fig:lip_expert_architecture}
  % \vspace{-0.1cm}
\end{figure}
The face mesh is obtained by adding the mean shape to the product of the expression parameters and expression bases.
\cref{fig:lip_expert_architecture} shows the architecture of the audio embedder and the mouth embedder. Both embedders incorporate a ReLU layer as their final layer to ensure the output remains positive. This guarantees that the cosine similarity of the outputs falls within the valid probability range of $[0, 1]$.


\subsubsection{Style Predictor}
The style predictor is implemented as a transformer encoder comprising six 8-head transformer encoder layers, each with a hidden size of $256$. The input features are all linearly projected to $256$.

\subsection{Data Details}
\subsubsection{Datasets}

\noindent\textbf{MEAD.} The dataset, an in-lab talking-face corpus, features 60 speakers articulating eight emotions at three different intensity levels. When dividing the MEAD dataset into training and test subsets, we adhere to previously established methodologies~\cite{ji2022eamm}.

\noindent\textbf{HDTF.}
The dataset stands out as a high-resolution, in-the-wild audio-visual dataset. We designate $10\%$ of HDTF videos for testing and reserve the remainder for training.

\noindent\textbf{Voxceleb2.}
Voxceleb2 is a large-scale talking head dataset with videos collected from YouTube. We redownload and recrop the videos to improve their resolution to $256\times256$. Subsequently, approximately $80000$ high-quality videos are selected, with $400$ allocated for testing and the rest for training.

\noindent\textbf{RAVDESS.}
The dataset features 24 professional actors (12 female, 12 male) vocalizing two 
lexically matched statements in a neutral North American accent. It encompasses a range of expressions in both speech and song, each articulated at two levels of emotional intensity, with an additional neutral expression included. We employ the speech data from RAVDESS, encompassing eight emotions, for evaluation.
% For style predictor, The division of training and test sets on the MEAD dataset aligns with the procedure employed for \method. 

\subsubsection{Data Processing}
The original videos are cropped and resized to $256\times256$ pixels, aligning with the specifications in FOMM \cite{siarohin2019first}, and are sampled at 25 FPS. The 3DMM parameters are extracted by Deep3DFace~\cite{deng2019accurate}.

Regarding the audio features used in the denoising network and the style-aware lip expert, we downsample the speech wave into the sampling rate of 16000 and extract acoustic features employing a pre-trained Wav2Vec2.0 model~\cite{baevski2020wav2vec}.

For audio features used in the style predictor, we extract them using a pre-trained HuBERT model~\cite{hsu2021hubert}. Besides, we also utilize low-level audio features including Mel Frequency Cepstrum Coefficients (MFCC), Mel-filterbank energy features (FBANK), fundamental frequency, and voice flag. These two type of features are concatenated to represent the audio features used in the style predictor.

\subsection{Evaluation Details}

\subsubsection{Style Accuracy Metric}
\label{sec:style_accuracy_metric}
The style classifier used in Style Accuracy (SA) is applied to 3DMM face motions. We evaluate this metric on MEAD only since the number of RAVEDESS videos for each style is inadequate to train a style classifier. We put the videos from the same speaker, emotion, and intensity into one style and train a style classifier to classify which style a face motion sequence belongs to. The style classifier is constructed mainly using 1D-CNNs.  For methods that do not generate 3DMM, we extract 3DMM from their results for evaluation.


\subsection{Training Details}

Our framework is implemented on Pytorch. We employ Adam~\cite{kingma2014adam} for optimization, with a learning rate set to $0.0001$. The number of diffusion steps for the denoising network and style predictor is $1000$. The training batch size for the denoising network, style predictor, and lip expert is $64$, $64$, and $32$, respectively. $\lambda_{\text{denoise}}$, $\lambda_{\text{sync}}$, $n$, and $w$ are set to $1$, $1$, $5$, and $5$, respectively. The number of frames for style reference and audio used in style prediction is limited to $64 - 256$, corresponding to a time length of $2.56 - 10.24$ seconds. The denoising network, style predictor, and lip expert are trained on one NVIDIA Tesla A100 GPU for about $3$, $1$, and $10.5$ hours, respectively.

\subsubsection{Finetuning PIRender}
The renderer is fine-tuned with the losses in ~\cite{ren2021pirenderer} using MEAD. Instead of training with the self-reconstruction protocol where the source frame and target frame are from the same video, we select the source frame and target frame from the same speaker with different emotions. This enables the renderer to generate emotions different from the input portrait. This also allows our method to utilize portraits with emotions, unlike previous approaches that are confined to using neutral portraits~\cite{ji2022eamm}. We incorporate some neutral videos in Voxceleb into the data used for fine-tuning, which enhances the performance in identity preservation.

% \subsubsection{Training Style-aware Lip Expert}
% The style-aware lip expert is trained to discriminate whether the input audio and face motions are synchronized. We use cosine-similarity with binary cross-entropy loss to train the lip expert. Specifically, we compute cosine-similarity for the face motion embedding $\vect{e}^m$ and audio embedding $\vect{e}^a$ to represent the probability that the input audio-motion pair is synchronized. The training loss of the lip expert is: 
% \begin{equation}
%     \mathcal{L}_{\eqword{expert}} =\eqword{BCE}( \frac{\vect{e}^m\cdot \vect{e}^a}{\max (||\vect{e}^m||_2\cdot||\vect{e}^a||_2 , \epsilon )}),
% \end{equation}
% where $\epsilon$ is a small number for avoiding the division-by-zero error.

\subsection{Inference Details}
The inference of the denoising network can be accelerated with DDIM. We generate samples with $10$ DDIM steps and observe no performance drop. Generating a 30-second video offline takes $15.61$ seconds, with the face motion generation only taking $1.24$ seconds. During evaluation, the scale factor $\omega$ of classifier-free guidance is set to $1$. The style predictor uses the sampling algorithm of DDPM to predict style codes.

The emotion conveyed in the style reference (video or audio), should remain consistent to avoid confusing the model.

The head pose information, which is fed into the renderer, can be derived from real videos or generated using existing methods~\cite{wang2021audio2head}.


==> supp_sec/04_applications.tex <==
\section{Applications}

Talking head for ChatGPT.
apply to other facial 3DMM and avatar
\todo{refer to GestureDiffuCLIP and MakeItTalk}

==> supp_sec/05_limitations_and_future_work.tex <==
\section{Limitations}

% Although our method has achieved promising results in expressive talking head generation, it still has a few limitations that present novel research opportunities.

% Firstly, our method may produce artifacts(teeth flickering) around the mouth when generating intense expressions. Generating teeth is a long-standing challenge in talking head generation since the algorithm needs to inpaint the teeth area that are often occluded in the input portrait. Since under intense expressions, the teeth area is bigger. The issue becomes worse. The issue can be solved by incorporating modules~\cite{lv2022generating,ye2022dynamic,li2023hdtr} proposed recently that enhance the teeth quality. A more thoroughly solution is to devise a renderer specific to emotional talking head generation. Existing renderers~\cite{xu2023high,ma2023styletalk,gan2023efficient,ji2022eamm} are mainly adapted from existing facial reenactment methods with little change. An emotion-aware renderer will not only generate good teeth area, but also enhance the generation of vivid emotions.

% Secondly, our method do not produce speaking styles that are varied with time. In real-world scenarios, the speaking style of speaker is changing as time goes. Our method do not capture this characteristic. A typical impact on results is that when the speech is end, our method still generate face with somewhat intense emotions(wide-open mouth when surprised) but not face with a close mouth. The solution is to introduce a module that predicts speaking style as time goes.

% Thirdly, we observe that the style predictor struggles to predict correct emotions for some audio clips in MEAD with low emotion intensity (\eg some audio in MEAD intensity level1 video). We observe that the emotion conveyed these audio clips is very similar to neutral emotion and thus confusing the prediction. We also observed that although the videos in the MEAD dataset clearly express emotions due to the good training and supervision of the speakers, sometimes the audio does not correspond with the emotions that should be expressed. Therefore, one solution to increase prediction accuracy is to use a better dataset. Another solution is to incorporate the text information in audio during speaking style prediction, which is a common practice in speech emotion recognition~\cite{wang2023exploring,chen2022key}.

% Despite these limitations, DreamTalk represents a significant step towards generating high-quality results in expressive talking head generation.

% ---

Despite DreamTalk's promising advancements in emotional talking head generation, it encounters several challenges that open avenues for future research.

When using a constant style reference, DreamTalk generates expressions that are strictly consistent with the main expressions in the reference but lack expression changes over time, such as eye blinking. Generating emotions with rich temporal variations is, compared to methods that generate neutral or coarse-grained emotions, more difficult for methods that achieve fine-grained emotional control, like DreamTalk. This is because these methods must achieve both precise control of expressions and diverse changes. To address the issue, temporal changes in expressions can be achieved by using temporally changing style references when generating each video frame. As discussed in \cref{sec:style_code_interpolation}, DreamTalk can achieve smooth expression changes by changing the style references.  Eye blinks can be achieved by using eye blink loss~\cite{zhang2023sadtalker} during training or post-editing 3DMM, a common practice used in previous methods~\cite{cudeiro2019capture,peng2023emotalk} that also aim to control expressions. Specifically, we can obtain the parameter changes of blinking and then edit the generated expression parameters. A video with the eye blinking through post-editing is shown in \suppvideo.

DreamTalk may change the speaker's identity when the identity in the reference video highly differs from that in the portrait. The reason is that 3DMM expression parameters leak identity information. This leakage leads to the generated identity becoming somewhat similar to the identity in the reference. The issue can be mitigated by adopting 3DMM which decouples expression and identity information more effectively.

The style predictor sometimes struggles with accurately identifying emotions in low-emotion-intensity audio clips from the MEAD dataset. The reason is that in some MEAD videos, the audio does not correspond with the expressed emotions. To enhance prediction accuracy, it is beneficial to employ a dataset where the audio closely aligns with the expressed emotions. Another solution is to incorporate textual information from audio during prediction, a strategy commonly employed in speech emotion recognition~\cite{wang2023exploring,chen2022key}.

DreamTalk occasionally produces artifacts around the mouth area, such as teeth flickering, particularly during intense expressions. The issue comes from the renderer and can be mitigated by using more advanced renderers or incorporating modules~\cite{lv2022generating,ye2022dynamic,li2023hdtr} proposed recently that enhance the teeth quality.

Despite these challenges, DreamTalk marks a significant stride in the realm of emotional talking head generation, paving the way for further innovations.

% Although our method has achieved promising results in text-guided speaking style control, it still has a few limitations that present novel research opportunities. Firstly, TalkCLIP struggles to generate correct speaking styles for texts that are too abstract, such as idioms (e.g., TalkCLIP failed to generate a happy speaking style for the text "He was over the moon about the ratings"). Secondly, TalkCLIP utilizes texts to control speaking styles while disregarding the emotion conveyed in the audio, which could result in inconsistencies between the generated videos and input audio emotions. Additionally, our method may produce artifacts around the mouth when generating intense expressions, and we aim to explore more advanced rendering techniques in future research. 



==> supp_sec/06_ethical_consideration.tex <==
\section{Ethical Consideration}

\method is able to generate realistic talking head videos. This positions \method with a broad spectrum of potential applications, each carrying intricate societal implications. While \method holds significant potential in amplifying and enriching human creative endeavors and may pave the way for innovative tools for creative professionals, its capabilities also harbor risks. There's a possibility for \method to generate content that might encompass or imply sexual themes, promote hatred, or depict violence. Misuse of \method could lead to negative repercussions on individuals or groups, potentially erasing or maligning them, perpetuating stereotypes, and subjecting them to disrespect. Other concerns include the potential for harassment, intimidation, or exploitation. Furthermore, \method's capabilities might be harnessed to mislead or spread misinformation.

Before releasing \method, we have implemented and plan to introduce several safeguards to curb potential misuse. Users will be advised against using images without the depicted individuals' consent to combat harassment and bullying. To prevent the spread of misinformation, all \method outputs will bear watermarks indicating their synthetic nature. Our commitment remains steadfast in continuously researching ways to minimize adverse societal effects.

==> supp_sec/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}

\usepackage{colortbl} 
% \usepackage{xcolor}
\newcommand\wx[1]{{\color{blue}#1}}
\newcommand\zsw[1]{{\color{orange}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{cleveref}

\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{subcaption}
\usepackage{multirow}
%\usepackage{gensymb}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amssymb}
%\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{bm}

\usepackage[T1]{fontenc}
\usepackage{indentfirst} % added by wx


\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
\newcommand{\vect}[1]{\bm{#1}}

\usepackage{booktabs}
% \usepackage{natbib}
\usepackage{xspace}

\newcommand{\method}{DreamTalk\xspace}
% \newcommand{\stylespec}{style predictor\xspace}

\newcommand{\eqword}[1]{{\text{#1}}}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\absvalue}[1]{\lvert #1 \rvert}


\newcommand{\fig}{Figure{}~}
\newcommand{\eqn}{Equation{}~}

\newcommand{\supp}{\textit{Supp. Mat.}\xspace}
\newcommand{\suppvideo}{\textit{Supp. Video}\xspace}

\usepackage{pifont}
\usepackage{makecell}
\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
  \global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\small}
